On the Analysis of Quantum Repeater Chains with Sequential Swaps

We evaluate the performance of two-way quantum repeater chains with sequential entanglement swapping. Within the analysis we consider memory decoherence, gate imperfections, and imperfect link-level entanglement generation. Our main results include closed-form expressions for the average entanglement fidelity of the generated end-to-end entangled states. We generalize previous findings for the one-shot fidelity analysis and study the case where repeater chains serve end-to-end requests continuously. We provide solutions to the continuous request scenario by combining results from quantum information theory and queuing theory. Finally, we apply the formulas obtained to analyze the impacts of hardware parameters, i.e., coherence times and gate fidelity, and distance on the entanglement fidelity and secret key rate of homogeneous quantum repeater chains.

==> src/expectedState.tex <==
\section{Analysis of Entanglement distribution}

We now utilize \eqref{eq:dephasedCatBellPair} and \eqref{eq:depolarizedCatBellPair} to compute the expected entangled state distributed after a sequence of \ac{BSM} operations are performed when the time defining decoherence channels are considered to be random variables. Our results extend initial investigations for the fidelity of teleportation in a single quantum node~\cite{chandra2022scheduling} to the scenario of \ac{e2e} entanglement distribution. Let $T_j$ denote the random variable that denotes the time the decoherence channel $\mathcal{E}_j$ acts on the $j$-th Bell pair. The expected state for the case of dephasing and depolarizing noise is
\begin{align}
    & \mathbb{E}[\rho_{BSM}] = \frac{1 + M[X]}{2} \Phi + \frac{1 - M[X]}{2} \sigma \Phi \sigma,\label{eq:averageState}
\end{align}
and
\begin{align}
    & \mathbb{E}[\rho_{BSM}] = M[X] \Phi + (1 - M[X]) \frac{\mathbb{1}}{4},\label{eq:averageState},
\end{align}
respectively, where $M[X]$ is the moment generating function for the random variable $X = \sum_{j=1}^{n}-\tau_j T_j$. In the case of depolarizing, the expected state is given by


==> src/outline.tex <==
\begin{enumerate}
    \item Introduction
    \item Background / System model
    \begin{enumerate}
        \item Quantum network characterization: describe the network model, assuming probabilistic link-level entanglement generation and deterministic entanglement swapping operations.
        \item Connectionless 1st Gen Routing: Discuss entanglement generation in a "packet switching" network. Classical information propagates together with quantum information at each hop. Service decision based exclusively on local meta information contained in packets (e.g., based threshold fidelity)
        \item Queuing Theory model: abstract entanglement generation with exponential and request generation Poisson.
        \item Flow control mechanisms: discuss what are the impacts of flow control assuming that classical flow control is used to control rate in the quantum connectionless architecture. We'll essentially state that one can assume buffers are always full and you have an infinite request stream which is served on a rate specified by the congestion mechanism.
        \item Continuous-time quantum channels for decohernce: define channels that can be expressed in exponential form in continuous time (depolarizing, dephasing, and amplitude damping).
        \item Gate noise model: describe a noise model for Bell state measurements. This can be done by modeling the error on a CNOT gate + qubit measurements. Gate errors can be factored out under the assumption of teleportation covariance of our operations. This is true for depolarizing and dephasing channels for sure.
    \end{enumerate}
    \item Performance analysis under Poisson arrivals
    \begin{enumerate}
        \item Show derivation of average fidelity for Poisson arrivals and exponential service time for an arbitrary length chain, including gate errors. \textcolor{blue}{Contribution: show that queues in tandem allow for calculating distributed fidelity for chains.}
        \item Provide closed form expressions for depolarizing, dephasing, amplitude damping, and possible combinations of the channels.
        \item \textcolor{red}{Analyse performance with physical distance rather than hop-distance alone.}
        \item \textcolor{red}{Link-level distillation: It should be possible to model link-level distillation here. We can simply assume that we have a slower process leading to a higher fidelity and try to compare how rate changes by doing so. What is interesting is that we are playing with the fidelity-rate tradeoff without changing pump power. Depending on the form of the solution, we could try to find an optimal operating point.}
    \end{enumerate}
    \item Performance analysis for equilibrium state in flow control.
    \begin{enumerate}
        \item Show derivation of average fidelity when congestion control is performed in the system. \textcolor{blue}{Contribution: extend the results presented in Section 3, which now also work for discrete-time service processes under the assumption that congestion control works.}
        \item Provide closed form expressions for depolarizing, dephasing, amplitude damping, and possible combinations of the channels.
        \item Matheus suggestion: Repeat here points 3-c) and 3-b).
    \end{enumerate}
    \item Bottleneck analysis: We can utilize the descriptions we had previously to analyse the effects of different hardware parameters into delivered fidelity.
    \begin{enumerate}
        \item Find operation point for link-level distillation such that average fidelity is higher than 0.81 (distillable entanglement). \textcolor{blue}{Contribution: Demonstrate that connectionless, one-way-like entanglement distribution protocols can be used to serve useful entanglement.} 
        \item Coherence time vs gate noise---studying effects with distance. Analyse for different distance regimes, the effects of coherence time and initial fidelities into the average distributed fidelity. \textcolor{blue}{Contribution: understand which of these two should be prioritized based on network distance.} 
    \end{enumerate}
    \item Conclusion
\end{enumerate}
